Learning Decentralized Flocking Controllers with Spatio-Temporal Graph Neural Network

Recently a line of researches has delved the use of graph neural networks (GNNs) for decentralized control in swarm robotics. However, it has been observed that relying solely on the states of immediate neighbors is insufficient to imitate a centralized control policy. To address this limitation, prior studies proposed incorporating $L$-hop delayed states into the computation. While this approach shows promise, it can lead to a lack of consensus among distant flock members and the formation of small clusters, consequently resulting in the failure of cohesive flocking behaviors. Instead, our approach leverages spatiotemporal GNN, named STGNN that encompasses both spatial and temporal expansions. The spatial expansion collects delayed states from distant neighbors, while the temporal expansion incorporates previous states from immediate neighbors. The broader and more comprehensive information gathered from both expansions results in more effective and accurate predictions. We develop an expert algorithm for controlling a swarm of robots and employ imitation learning to train our decentralized STGNN model based on the expert algorithm. We simulate the proposed STGNN approach in various settings, demonstrating its decentralized capacity to emulate the global expert algorithm. Further, we implemented our approach to achieve cohesive flocking, leader following and obstacle avoidance by a group of Crazyflie drones. The performance of STGNN underscores its potential as an effective and reliable approach for achieving cohesive flocking, leader following and obstacle avoidance tasks.

==> sections/0authers.tex <==
%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
% \author{Siji Chen}
% % \authornote{Both authors contributed equally to this research.}
% \orcid{0009-0009-1691-0600}
% \affiliation{%
%   \institution{Virginia Tech}
%   % \streetaddress{P.O. Box 1212}
%   \city{Falls Church}
%   \state{VA}
%   \country{USA}
%   % \postcode{43017-6221}
% }
% \email{sijic@vt.edu}

% \author{Yanshen Sun}
% \affiliation{%
%   \institution{Virginia Tech}
%   % \streetaddress{P.O. Box 1212}
%   \city{Falls Church}
%   \state{VA}
%   \country{USA}
%   % \postcode{43017-6221}
% }
% \email{yansh93@vt.edu}

% \author{Peihan Li}
% \affiliation{%
%   \institution{Drexel University}
%   \city{Philadelphia}
%   \state{PA}
%   \country{USA}
% }
% \email{pl525@drexel.edu}

% \author{Lifeng Zhou}
%  \affiliation{%
%   \institution{Drexel University}
%   \city{Philadelphia}
%   \state{PA}
%   \country{USA}
% }
% \email{lz457@drexel.edu}

% \author{Chang-Tien Lu}
% \affiliation{%
%   \institution{Virginia Tech}
%   \city{Falls Church}
%   \state{VA}
%   \country{USA}
%   % \postcode{43017-6221}
% }
% \email{ctlu@vt.edu}

%\author{TBD$^{1}$,$^{2}$% <-this % stops a space
\author{Siji Chen, Yanshen Sun, Peihan Li, Lifeng Zhou, Chang-Tien Lu % <-this % stops a space
\thanks{Virginia Tech, Drexel University, Philadelphia, PA 19104, USA. Email: \texttt{\small \{sijic@vt.edu, yansh93@vt.edu, pl525@drexel.edu, lz457@drexel.edu, ctlu@vt.edu\}}.}
% \thanks{$\dagger$These authors contributed equally.}%
